Chaos synchronization: Using prey abundance to synchronize two chaotic GLV models

This work investigates the synchronization between two chaotic food webs using the generalized Lotka-Volterra (GLV) model consisting of one prey and two predator populations. We, first, examine the impact of three functional responses (linear, Holling type II, and Holling type III) on system dynamics For the study, we consider the model with a linear functional response consisting of chaotic oscillations and apply controllers to stabilize its unstable fixed points. This research contributes to the understanding of how to apply chaotic ecological models to predict the population of competing species in one habitat using information about similar populations in another system. To do this, we configure a drive-response system where prey acts as the driving variable and both predators depend only on the prey. We use active and adaptive control methods to synchronize two coupled GLV models and verify the analytical results through numerical simulations.

==> bbl.tex <==
\begin{thebibliography}{}
%
% and use \bibitem to create references. Consult the Instructions
% for authors for reference list style.
%
\bibitem{RefJ}
% Format for Journal Reference
Author, Article title, Journal, Volume, page numbers (year)
Wiggins, Stephen,Introduction to applied nonlinear dynamical systems and chaos,Springer Science \& Business Media,2003.
\bibitem
Pecora, Louis M and Carroll, Thomas L, Synchronization in chaotic systems, APS, 64, 821(1990).
\bibitem 
Nightingale, Edmund B and Veeraraghavan, Kaushik and Chen, Peter M and Flinn, Jason, Rethink the sync, ACM Transactions on Computer Systems (TOCS), 26,6 (2008).
\bibitem 
Chen, Shihua and L{\"u}, Jinhu, Synchronization of an uncertain unified chaotic system via adaptive control, Pergamon, 14, 643--647 (2002).

\bibitem 
Pecora, Louis M and Carroll, Thomas L,Master stability functions for synchronized coupled systems, Physical review letters (APS), 80,10 (1998)
\bibitem
Elsadany, AA and Matouk, AE and Abdelwahab, AG and Abdallah, HS, Dynamical analysis, linear feedback control and synchronization of a generalized Lotka-Volterra system, International Journal of Dynamics and Control (Springer), 6,  328--338 (2018).
\bibitem
Ackleh, Azmy S and Marshall, David F and Heatherly, Henry E, Extinction in a generalized Lotka-Volterra predator-prey model, International Journal of Stochastic Analysis (Hindawi Publishing Corporation), 13, 287--297 (1900).
\bibitem 
Malcai, Ofer and Biham, Ofer and Richmond, Peter and Solomon, Sorin,heoretical analysis and simulations of the generalized Lotka-Volterra model, Physical Review E (APS), 66, 3 (2002).

\bibitem{feng2005adaptive}
Feng, Jianwen and Chen, Shihua and Wang, Changping, Adaptive synchronization of uncertain hyperchaotic systems based on parameter identification, Chaos, Solitons \& Fractals (Elsevier),26,1163--1169 (2005).

\bibitem{vaidyanathan2015anti}
Vaidyanathan, Sundarapandian,Anti-synchronization of the generalized Lotka-Volterra three-species biological systems via adaptive control,International Journal of PharmTech Research, 8, 141--156 (2015).  
\bibitem{vaidyanathan2015global}
Vaidyanathan, Sundarapandian, Global chaos synchronization of the Lotka-Volterra biological systems with four competitive species via active control, International Journal of PharmTech Research, 8, 206--217 (2015).

\bibitem{vaidyanathan2016hybrid}
Vaidyanathan, Sundarapandian,Hybrid synchronization of the generalized Lotka-Volterra three-species biological systems via adaptive control,Int J PharmTech Res, 9, 179--192 (2019).
\bibitem{zheng2017simple}
Zheng, Jiming and Li, Xiaoshuang and Qiu, Yang, A Simple Hybrid Synchronization for a Class of Chaotic Financial Systems, Discrete Dynamics in Nature and Society, Hindawi, 2017 (2017).
\bibitem{hsu2005survey}
Hsu, Sze-Bi and others, A survey of constructing Lyapunov functions for mathematical models in population biology, Taiwanese Journal of Mathematics, The Mathematical Society of the Republic of China, 9, 151--173 (2005).
\bibitem{wolf1985determining}
Wolf, Alan and Swift, Jack B and Swinney, Harry L and Vastano, John A, Determining Lyapunov exponents from a time series, Physica D: Nonlinear Phenomena, Elsevier, 16, 285--317 (1985).
\bibitem{das2014occurrence}
Das, Krishnapada and Samanta, Sudip and Biswas, Barasha and Chottapadhyay, Joydev, Occurrence of chaos and its possible control in a predator-prey model with disease in the predator population, The Journal of Ecology, 108, 306--319 (2014).
\bibitem{kramer2013spatially}
Kramer, Sean and Bollt, Erik M, Spatially dependent parameter estimation and nonlinear data assimilation by autosynchronization of a system of partial differential equations, Chaos: An Interdisciplinary Journal of Nonlinear Science, AIP 23, 3, 033101 (2013).
\bibitem{singh2010synchronization}
Singh, Anuraj and Gakkhar, Sunita,ynchronization of chaos in a food web in ecological systems,World Academy of Science, Engineering and Technology, 70, 94--98 (2010).
\bibitem{wu2010chaos}
Wu, Xiang-Jun and Li, Jie and Upadhyay, Ranjit Kumar, Chaos control and synchronization of a three-species food chain model via Holling functional response,  International Journal of Computer Mathematics, Taylor \& Francis, 87,1, 199--214 (2010).
\bibitem{upadhyay1997chaos}
Upadhyay, Ranjit Kumar and Rai, Vikas, Why chaos is rarely observed in natural populations, Elsevier, 8,12, 1933-1939 (1997).
\bibitem{samardzija1988explosive}
amardzija, Nikola and Greller, Larry D, Explosive route to chaos through a fractal torus in a generalized Lotka-Volterra model, Bulletin of Mathematical Biology, Springer, 50,5, 465--491 (1988).
\bibitem{rao1999global}
Rao, V Sree Hari and Phaneendra, Bh RM, Global dynamics of bidirectional associative memory neural networks involving transmission delays and dead zones, Neural networks, Elsevier, 12,3, 455--465 (1999).
\bibitem{zhang2001global}
Zhang, Jiye and Yang, Yiren, Global stability analysis of bidirectional associative memory neural networks with time delay, Wiley Online Library, 29, 2, 185--196 (2001).
\bibitem{yassen2006adaptive}
Yassen, MT,Adaptive chaos control and synchronization for uncertain new chaotic dynamical system, Elsevier, Physics Letters A, 350, 1-2, 36--43 (2006).
\bibitem{cai2006adaptive}
Cai, Guoliang and Huang, Juanjuan and Tian, Lixin and Wang, Qingchao, Adaptive control and slow manifold analysis of a new chaotic system, International Journal of Nonlinear Science, 2, 1, 50--60 (2006).
\bibitem{min2007barbalat}
Min, Ying-Ying and Liu, Yun-Gang, Barbalat lemma and its application in analysis of system stability, Journal of Shandong University (engineering science), 37, 1, 51--55 (2007).
\bibitem{patidar2002synchronization}
Patidar, Vinod and Sud, KK, Synchronization in chaotic jerk dynamical systems, Indian Journal of Physics, 76, 553--557 (2002).
\bibitem{rangarajan1998lyapunov}
  Rangarajan, Govindan and Habib, Salman and Ryne, Robert D, Lyapunov exponents without rescaling and reorthogonalization},Physical Review Letters, APS, 80, 17, 3747 (1998). 
  
\bibitem{meador2011numerical}
 Meador, Clyde-Emmanuel Estorninho, Numerical calculation of Lyapunov exponents for three-dimensional systems of ordinary differential equations (2011).


\bibitem{Ginoux}
Ginoux, Jean-Marc, and Bruno Rossetto, Differential geometry and mechanics: applications to chaotic dynamical systems, International Journal of Bifurcation and Chaos 16, 887-910 (2006).

\bibitem{Yassen, M. T.}
Yassen, M. T., Adaptive control and synchronization of a modified Chua's circuit system, Applied Mathematics and Computation, 135, 113-128 (2003).

\bibitem{Pecora}
Pecora, Louis M., and Thomas L. Carroll, Synchronization in chaotic systems, Physical review letters 64.8: 821  (1990).

\bibitem{chen2002parameters}
Chen, Shihua and L{\"u}, Jinhu, Parameters identification and synchronization of chaotic systems based upon adaptive control, Physics Letters A, Elsevier, 299, 4, 353--358 (2002).
\bibitem{fotsin2005adaptive}
Fotsin, HB and Daafouz, J, Adaptive synchronization of uncertain chaotic colpitts oscillators based on parameter identification, Physics Letters A,Elsevier, 339, 3-5, 
\bibitem{lahav2018synchronization}
Lahav, Nir and Sendi{\~n}a-Nadal, Irene and Hens, Chittaranjan and Ksherim, Baruch and Barzel, Baruch and Cohen, Reuven and Boccaletti, Stefano, Synchronization of chaotic systems: A microscopic description, Physical Review E, APS 98, 5, 052204 (2018).

\bibitem{lorenz1963deterministic}
Lorenz, Edward N, Deterministic nonperiodic flow, Journal of the atmospheric sciences, 20, 2, 130--141 (1963).
\bibitem{luo2009theory}
Luo, Albert CJ, A theory for synchronization of dynamical systems, Communications in Nonlinear Science and Numerical Simulation, Elsevier, 14, 5, 1901--1951 (2009).

\bibitem{li1975period}
  Li, Tien-Yien and Yorke, James A, Period three implies chaos, The American Mathematical Monthly, Taylor \& Francis, 82, 10, 985--992 (1975).
\bibitem{hunt2015defining}
 Hunt, Brian R and Ott, Edward, Defining chaos,  Chaos: An Interdisciplinary Journal of Nonlinear Science, AIP Publishing, 25, 9, 097618 (2015).
 
\bibitem{pecora2015synchronization}
 Pecora, Louis M and Carroll, Thomas L, Synchronization of chaotic systems, Chaos: An Interdisciplinary Journal of Nonlinear Science,AIP Publishing, 25, 9, 097611 (2015).

\bibitem{{upadhyay2009complex}
Upadhyay, Ranjit Kumar and Rai, Vikas, Complex dynamics and synchronization in two non-identical chaotic ecological systems, Chaos, Solitons \& Fractals, Elsevier,  40, 5, 2233-2241 (2009).

\bibitem{park2005adaptive}
Park, Ju H, Adaptive synchronization of a unified chaotic system with an uncertain parameter,International Journal of Nonlinear Sciences and Numerical Simulation, De Gruyter, 6, 2, 201--206 (2005)
\bibitem{lu2005adaptive}
  Lu, Jianquan and Cao, Jinde, Adaptive complete synchronization of two identical or different chaotic (hyperchaotic) systems with fully unknown parameters}, Chaos: An Interdisciplinary Journal of Nonlinear Science, AIP, 15, 4, 043901 (2005).
\bibitem{kozlovski1998integral}
Kozlovski, OS, An integral formula for topological entropy of $ {C}^{\infty}$ maps,Ergodic theory and dynamical systems, Cambridge University Press, 18, 2, 405--424 (1998).
\bibitem{blasius1999complex}
 Blasius, Bernd and Huppert, Amit and Stone, Lewi, Complex dynamics and phase synchronization in spatially extended ecological systems,Nature, Nature Publishing Group, 399, 6734, 354(1999).
\bibitem{liu2003largest}
  Liu, Hai-Feng and Yang, Yong-Zhe and Dai, Zheng-Hua and Yu, Zun-Hong, The largest Lyapunov exponent of chaotic dynamical system in scale space and its application,
  Chaos: An Interdisciplinary Journal of Nonlinear Science, AIP, 13, 3, 839--844 (2003).
 \bibitem{RefB}

Solari, Hern{\'a}n G and Natiello, Mario A and Mindlin, Gabriel B, Nonlinear dynamics: a two-way trip from physics to math,CRC Press (1996).
\bibitem
Strogatz, Steven H,{Nonlinear dynamics and chaos: with applications to physics, biology, chemistry, and engineering,CRC Press (2018).
\bibitem{parlitz1999synchronization}
Parlitz, Ulrich and Junge, L, synchronization of chaotic systems, Control Conference (ECC), 1999 European, 4637--4642, IEEE (1999).
\bibitem{kramer2013oceanographic}
Kramer, Sean Jason, Oceanographic Modeling with Hyperspectral Satellite Imagery, Citeseer (2013).
\bibitem{verhulst2006nonlinear}
Verhulst, Ferdinand, Nonlinear differential equations and dynamical systems, Springer Science \& Business Media(2006).
\bibitem{simmons2016differential}
Simmons, George F,Differential equations with applications and historical notes, CRC Press (2016). 
\end{thebibliography}
